Distortion Reduction for Off-Center Perspective Projection of Panoramas

A single Panorama can be drawn perspectively without distortions in arbitrary viewing directions and field-of-views when the camera position is at the origin. This is a key advantage in VR and virtual tour applications because it enables the user to freely"look around" in a virtual world with just a single panorama, albeit at a fixed position. However, when the camera moves away from the center, barrel distortions appear and realism breaks. We propose modifications to the equirectangular-to-perspective(E2P) projection that significantly reduce distortions when the camera position is away from the origin. This enables users to not only "look around" but also "walk around" virtually in a single panorama with more convincing renderings. We compare with other techniques that aim to augment panoramas with 3D information, including: 1) panoramas with depth information and 2) panoramas augmented with room layouts, and show that our approach provides more visually convincing results

==> analysis.tex <==
\section{Analysis}
\label{sec:analysis}

TODO

\subsection{Computational dolly zoom effect analysis}
\label{sec:dolly_analysis}

TODO

\subsection{Ablation studies}
\label{sec:ablation}

TODO
